Foundation Models for Weather and Climate Data Understanding: A Comprehensive Survey

As artificial intelligence (AI) continues to rapidly evolve, the realm of Earth and atmospheric sciences is increasingly adopting data-driven models, powered by progressive developments in deep learning (DL). Specifically, DL techniques are extensively utilized to decode the chaotic and nonlinear aspects of Earth systems, and to address climate challenges via understanding weather and climate data. Cutting-edge performance on specific tasks within narrower spatio-temporal scales has been achieved recently through DL. The rise of large models, specifically large language models (LLMs), has enabled fine-tuning processes that yield remarkable outcomes across various downstream tasks, thereby propelling the advancement of general AI. However, we are still navigating the initial stages of crafting general AI for weather and climate. In this survey, we offer an exhaustive, timely overview of state-of-the-art AI methodologies specifically engineered for weather and climate data, with a special focus on time series and text data. Our primary coverage encompasses four critical aspects: types of weather and climate data, principal model architectures, model scopes and applications, and datasets for weather and climate. Furthermore, in relation to the creation and application of foundation models for weather and climate data understanding, we delve into the field's prevailing challenges, offer crucial insights, and propose detailed avenues for future research. This comprehensive approach equips practitioners with the requisite knowledge to make substantial progress in this domain. Our survey encapsulates the most recent breakthroughs in research on large, data-driven models for weather and climate data understanding, emphasizing robust foundations, current advancements, practical applications, crucial resources, and prospective research opportunities.

==> framework.tex <==
% \tikzstyle{my-box}=[
%     rectangle,
%     draw=hidden-draw,
%     rounded corners,
%     text opacity=1,
%     minimum height=1.5em,
%     minimum width=5em,
%     inner sep=2pt,
%     align=center,
%     fill opacity=.5,
%     line width=0.8pt,
% ]
% \tikzstyle{leaf}=[my-box, minimum height=1.5em,
%     fill=hidden-pink!80, text=black, align=left, font=\normalsize,
%     inner xsep=2pt,
%     inner ysep=4pt,
%     line width=0.8pt,
% ]
% \begin{figure*}[t]
%     \centering
%     \resizebox{1\textwidth}{!}{
%         \begin{forest}
%             forked edges,
%             for tree={
%                 fill=level0!80,
%                 grow=east,
%                 reversed=true,
%                 anchor=base west,
%                 parent anchor=east,
%                 child anchor=west,
%                 base=left,
%                 font=\large,
%                 rectangle,
%                 draw=hidden-draw,
%                 rounded corners,
%                 align=left,
%                 minimum width=4em,
%                 edge+={darkgray, line width=1pt},
%                 s sep=3pt,
%                 inner xsep=2pt,
%                 inner ysep=3pt,
%                 line width=0.8pt,
%                 ver/.style={rotate=90, child anchor=north, parent anchor=south, anchor=center},
%             },
%             where level=1{text width=9em,font=\normalsize,fill=level1!80,}{},
%             where level=2{text width=10em,font=\normalsize,fill=level2!80,}{},
%             where level=3{text width=10em,font=\normalsize,fill=level3!60,}{},
%             where level=4{text width=10em,font=\normalsize,}{},
%             % [
%                 Data-Driven Models for \\ Weather and Climate
%                 [
%                     Data-Driven Models \\ for Numerical Data
%                     [
%                         Foundation Models for \\ Weather and Climate
%                         [
%                             ClimaX~\cite{nguyen2023climax}, FourCastNet~\cite{pathak2022fourcastnet}, GraphCast~\cite{lam2022graphcast}, PanGu-Weather~\cite{bi2023accurate}, W-MAE~\cite{man2023w}, FengWu~\cite{chen2023fengwu}, leaf, text width=11.5em
%                         ]
%                     ]
%                     [
%                         PFMs for Time \\ Series Data
%                         [
%                         ]
%                         [
%                             Domain-Specific
%                             [
%                                 \textbf{Event Prediction:} PromptTPP~\cite{xue2023prompttpp}
%                                 , leaf, text width=17em
%                             ]
%                         ]
%                     ]
%                 ]
%                 [                
%                     Large Models for \\ Spatio-Temporal \\ Data (\shortautoref{sec: Large Models for Spatio-Temporal Data})
%                     [
%                         LLMs for Spatio-\\Temporal Data
%                         [
%                             Spatio-Temporal \\Graphs
%                             % [
%                             %     \textbf{Reasoning:} Graph-ToolFormer~\cite{zhang2023graph} 
%                             %     , leaf, text width=15em
%                             % ]
%                             [
%                                 \textbf{Action Recognition:}  LA-GCN~\cite{xu2023language}
%                                 , leaf, text width=17em
%                             ]
%                             [
%                                 \textbf{Finance:} Chen \textit{et al.}~\cite{chen2023chatgpt}
%                                 , leaf, text width=11.5em
%                             ]
%                         ]
%                         [
%                             Temporal \\Knowledge Graphs
%                             [
%                                 \textbf{Completion:} PPT~\cite{xu2023pre}{, } Chen \textit{et al.}~\cite{chen2023knowledge}
%                                 , leaf, text width=18.5em
%                             ]
%                             [
%                                 \textbf{Forecasting:} Lee \textit{et al.}~\cite{lee2023temporal}
%                                 , leaf, text width=12.5em
%                             ]
%                         ]
%                         [
%                             Video Data
%                             [
%                                 \textbf{Captioning:} Vid2Seq~\cite{yang2023vid2seq}
%                                 , leaf, text width=12em
%                             ]
%                             [
%                                 \textbf{Other Tasks:} VideoLLM~\cite{chen2023videollm}{, } Valley~\cite{luo2023valley}{, } \\Video-LLaMA~\cite{zhang2023video}{, } LAVILA~\cite{zhao2023learning}
%                                 , leaf, text width=19em
%                             ]
%                         ]
%                     ]
%                     [
%                         PFMs for Spatio-\\Temporal Data
%                         [
%                             Spatio-Temporal \\Graphs
%                             [
%                                 \textbf{Climate:} DLWP~\cite{weyn2020improving}{, } GraphCast~\cite{lam2022graphcast}{, } FourCastNet~\cite{pathak2022fourcastnet}{, } \\ClimaX~\cite{nguyen2023climax}{, }
%                                 FengWu~\cite{chen2023fengwu}{, }
%                                 Pangu-Weather~\cite{bi2023accurate}{, }
%                                 W-MAE~\cite{man2023w}
%                                 , leaf, text width=30em
%                             ]
%                             [
%                                 \textbf{Transportation:} CPPBTR~\cite{duan2019pre}{, }
%                                 % BDSTN~\cite{cao2021bert}{, }
%                                 TrafficBERT~\cite{jin2021trafficbert}{, }
%                                 TFM~\cite{wang2023building}
%                                 , leaf, text width=28em
%                             ]
%                         ]
%                         [
%                             Video Data
%                             [
%                                 \textbf{Multimodality:} mPLUG-2~\cite{xu2023mplug}
%                                 , leaf, text width=13.8em
%                             ]
%                         ]
%                       ]
%                     ]
%                 ]
%             ]
%         \end{forest}
%     }
%     % \vspace{-1mm}
% \caption{A comprehensive taxonomy of large models for time series and spatio-temporal data from the perspectives of methodologies (i.e., LLMs vs. PFMs), motivations (e.g., general vs. domain-specific purposes), and applications.}
% % \vspace{-4mm}
% \label{fig:Taxonomy}
% \end{figure*}
